Reset Controller Synthesis by Reach-avoid Analysis for Delay Hybrid Systems

A reset controller plays a crucial role in designing hybrid systems. It restricts the initial set and redefines the reset map associated with discrete transitions, in order to guarantee the system to achieve its objective. Reset controller synthesis, together with feedback controller synthesis and switching logic controller synthesis, provides a correct-by-construction approach to designing hybrid systems. However, time-delay is an inevitable factor in hybrid systems, which can degrade control performance and render verification certificates obtained by abstracting away time-delay invalid in practice. In this paper, we investigate this issue in a practical manner by taking time-delay into account. We propose an approach that reduces the synthesis of reset controllers to the generation of reach-avoid sets for the hybrid system under consideration, which can be efficiently solved using off-the-shell convex optimization solvers.

==> macros.tex <==
\RequirePackage{todonotes}

\newcommand{\hscomment}[1]{\todo[color=red!30,size=\small,fancyline,author=Han]{#1}}
\newcommand{\hscommentinline}[1]{\todo[inline,color=red!30,author=Han]{#1}}
\newcommand{\aths}{\colorbox{cyan!30}{\textbf{@Han}}}

\newcommand{\ljcomment}[1]{\todo[color=cyan!30,size=\small,fancyline,author=Liu]{#1}}

\newcommand{\znjcomment}[1]{\todo[color=green!25,size=\small,fancyline,author=ZNJ]{#1}}
\newcommand{\blkcomment}[1]{\todo[color=green!25,size=\small,fancyline,author=Jiyu]{#1}}
\newcommand{\blkcommentinline}[1]{\todo[inline,color=green!25,author=Jiyu]{#1}}
\newcommand{\atblk}{\colorbox{green!25}{\textbf{@Jiyu}}}

\newcommand{\sfcomment}[1]{\todo[color=green!30,size=\small,fancyline,author=shenghua]{#1}}
\newcommand{\sfcommentinline}[1]{\todo[inline,color=green!30,author=Han]{#1}}
\newcommand{\atsf}{\colorbox{green!30}{\textbf{@shenghua}}}


\renewcommand{\qed}{\hfill $\square$}
\newcommand{\cmark}{\ding{51}} % 对勾
\newcommand{\xmark}{\ding{55}} % 叉号


%--------------- Colorful text ----------------------%
\definecolor{myred}{HTML}{e41a1c}
\definecolor{myblue}{HTML}{377eb8}
\definecolor{mygreen}{HTML}{4daf4a}
\definecolor{mygray}{gray}{0.6}
\definecolor{myorange}{HTML}{ffa510}
\newcommand{\mgreen}[1]{\textcolor{mygreen}{#1}}
\newcommand{\morange}[1]{\textcolor{myorange}{#1}}
\newcommand{\mblue}[1]{\textcolor{myblue}{#1}}

\newcommand{\redparg}[1]{\color{purple}{#1}\color{black}}
\newcommand{\red}[1]{\textcolor{purple}{#1}}
\newcommand{\blueparg}[1]{\color{blue}{#1}\color{black}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{teal}{#1}}
%--------------- Some Set of Number -----------------%
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Realn}{\Real^n}
\newcommand{\StrictPosReal}{\mathbb{R}_{>0}}
\newcommand{\PosReal}{\mathbb{R}_{\geq 0}}

\newcommand{\Int}{\mathbb{Z}}
\newcommand{\PosInt}{\mathbb{Z}_{\geq 0}}
\newcommand{\Nat}{\mathbb{N}}

%---------------- Some Set of Function --------------%
\newcommand{\ContiFun}[2]{\mathcal{C}({#1},{#2})}
\newcommand{\nContiFun}[3]{\mathcal{C}^{#1}({#2},{#3})}
\newcommand{\ContiNorm}[1]{||{#1}||_{\mathcal{C}}}

\newcommand{\DefSym}{:=}

\newcommand{\Poly}[1]{\Real [{#1}]}
\newcommand{\SOSPoly}[1]{\Sigma[{#1}]}

%---------------- Mathematical Computation Symble -----------------%
\newcommand{\Partial}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\PowSet}[1]{\mathcal{P}({#1})}


%---------------- Mathamatical Symble for proof ------------------%
\newcommand{\st}{,\,s.t.~}


%----------------- Macros Specified for This Paper ---------------%
\newcommand{\x}{\bm{x}}
\newcommand{\y}{\bm{y}}
\newcommand{\f}{\bm{f}}
%\newcommand{\e}{\bm{e}}
\newcommand{\pphi}{\bm{\phi}}

\newcommand{\set}[1]{{#1}}
\newcommand{\fset}[1]{\mathcal{#1}}
\newcommand{\vect}[1]{\bm{#1}}

%====  Delay hybrid automata ====%
\newcommand{\DisState}{Q} % discrete state
\newcommand{\ContiState}{X} % continuous state
\newcommand{\Dom}{\ensuremath{I}} % invariance of each mode
\newcommand{\Init}{\textit{Init}} % initial set of dHA
\newcommand{\ContiDyn}{F} % continuous dynamics in each mode
\newcommand{\Guard}{G} % gurad condition for discrete jump
\newcommand{\DisJump}{E} % discrete jump
\newcommand{\STime}{\textit{ST}} % delay in each discrete jump
\newcommand{\Reset}{R} % reset map in each discrete jump

\newcommand{\edHAabb}{\mathtt{dHA}}
\newcommand{\edHA}{\bm{\mathcal{H}}~=~(\DisState,\ContiState,\Dom,\ContiDyn,\Init,\DisJump,\Guard,\STime,\Reset)}
\newcommand{\edHAsyb}{\bm{\mathcal{H}}}

\newcommand{\dom}[1]{\mathtt{Dom}({#1})} % invariance of each mode
\newcommand{\dyn}[1]{\vect{f}_{#1}} % continuous dynamics in each mode
\newcommand{\guard}[1]{\set{G}({#1})} % gurad condition for discrete jump
\newcommand{\disjump}[2]{({#1},{#2})} % discrete jump
\newcommand{\eqdisjump}[2]{\vect{e}=({#1},{#2})} % discrete jump
\newcommand{\swittime}[1]{T({#1})} % delay in each discrete jump
\newcommand{\reset}[2]{R({#1},{#2})} % reset map in each discrete jump


%===== delay differential equation with barrier functional ======%
\newcommand{\cdds}{(\Init,\f,\Dom)}

\newcommand{\Usafe}{U}
\newcommand{\Safe}{S}
\newcommand{\fsafe}{s}
\newcommand{\ftarget}{g}
\newcommand{\Target}{T}
\newcommand{\domain}{D}
\newcommand{\oomit}[1]{}

\newcommand{\RA}{\mathcal{R\!\!A}}
\newcommand{\R}{\mathcal{R}_{\edHAsyb}}

%=====  Nodeterministic Finite Automata =====%
\newcommand{\NFA}{\mathtt{NFA}}
\newcommand{\DG}{\mathtt{DG}}

\newcommand{\InnerRA}[3]{\mathtt{InRA}\,(\,{#1},\,{#2},\,{#3})}
\newcommand{\ModeSeg}[3]{\mathtt{ModePartition}\,(\,{#1},\,{#2},\,{#3})}

\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother


\newcommand{\TAG}[1]{{\tag*{\small{[{#1}]}}}}

==> tikz.tex <==
\RequirePackage{tikz}
\RequirePackage{pgfplots}

\usetikzlibrary{
	cd,
	math,
	decorations.markings,
	decorations.pathreplacing,
	positioning,
	arrows.meta,
	circuits.logic.US,
	shapes,
	calc,
	fit,
	quotes,
  scopes,
  patterns,
  backgrounds}

\usepgfplotslibrary{groupplots, fillbetween}



\pgfplotsset{
  Axis Set/.style = {
    axis lines=middle,
    axis equal,
    axis line style = {mygray},
    clip=false,
		every axis y label/.style={
			at={(ticklabel* cs:1)},
			anchor=west,
            color=mygray,
		},
        every axis x label/.style={
			at={(ticklabel* cs:1)},
			anchor=south,
            color=mygray,
		},
        tick label style={mygray},
        yticklabel style={yshift=0.5ex},
		%			footnotesize,
		width = 6.5cm, %% As big as this example can be without spilling over onto the next slide
		height = 4cm, %% ditto
		%			ticks = none,
		xtick = {1,2,3,4},
    %ytick = {1,2,3,4,5},
    xmin = 0, 
    ymin = 0
  }
}
